A severe local flood and social events show a similar impact on human mobility

While a social event, such as a concert or a food festival, is a common experience to people, a natural disaster is experienced by a fewer individuals. The ordinary and common ground experience of social events could be therefore used to better understand the complex impacts of uncommon, but devastating natural events on society, such as floods. Based on this idea, we present a comparison - in terms of human mobility -, between an extreme local flood that occurred in 2017 in Switzerland, and social events which took place in the same region, in the weeks before and after the inundation. Using mobile phone location data, we show that the severe local flood and social events have a similar impact on human mobility, both at the national scale and at a local scale. At the national level, we found a small difference between the distributions of visitors and their travelled distances among the several weeks in which the events took place. At the local level, instead, we detected the anomalies (in time series) in the number of people travelling each road and railway, and we found that the distributions of anomalies, and of their clusters, are comparable between the flood and the social events. Hence, our findings suggest that the knowledge on ubiquitous social events can be employed to characterise the impacts of rare natural disasters on human mobility. The proposed methods at the local level can thus be used to analyse the disturbances in complex spatial networks and, in general, as complementary approaches for the analyses of complex systems.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
